On the Age of Information of Short-Packet Communications with Packet Management

In this paper, we consider a point-to-point wireless communication system. The source monitors a physical process and generates status update packets according to a Poisson process. The packets are transmitted to the destination by using finite blocklength coding to update the status (e.g., temperature, speed, position) of the monitored process. In some applications, such as real-time monitoring and tracking, the timeliness of the status updates is critical since the users are interested in the latest condition of the process. The timeliness of the status updates can be reflected by a recently proposed metric, termed the age of information (AoI). We focus on the packet management policies for the considered system. Specifically, the preemption and discard of status updates are important to decrease the AoI. For example, it is meaningless to transmit stale status updates when a new status update is generated. We propose three packet management schemes in the transmission between the source and the destination, namely non-preemption (NP), preemption (PR) and retransmission (RT) schemes. We derive closed-form expressions of the average AoI for the proposed three schemes. Based on the derived analytical expressions of the average AoI, we further minimize the average AoI by optimizing the packet blocklength for each status update. Simulation results are provided to validate our theoretical analysis, which further show that the proposed schemes can outperform each other for different system setups, and the proposed schemes considerably outperform the existing ones without packet management at medium to high generation rate.

==> retransmission.tex <==
\section{Performance Analysis of AoI with Retransmission}
We now study the average AoI of the system under retransmission scheme. We investigate the retransmission scheme that the IoT device keeps retransmitting the current update until it is successfully decoded by the destination or it is preempted by a new update. Note that the retransmission scheme for the non-preemption model is inefficient as the IoT device has to finish the service of the current status update before starting the service of a new update, even if it has already spend a long time on the current update. The evolution of AoI for the considered retransmission scheme is depicted in Fig. \ref{fig:queueing3}. We subsequently evaluate the three terms ${\mathbb {E}\left\{ {{Y_i^2}} \right\}}$, ${\mathbb {E}\left\{ {{Y_i}} \right\}}$ and ${\mathbb {E}\left\{ {{S_i}} \right\}}$ of the considered retransmission scheme in order to derive the average AoI.

First of all, different from the non-retransmission scheme studied in Section III that the service time is a fixed value $M$, the service time of the retransmission scheme is a multiple of $M$. We now characterize the expectation of $S_i$ for the retransmission scheme. Specifically, as a update may be dropped during retransmission if it is preempted by a new update, the expectation of $S_i$ can be characterized as ${\mathbb {E}\left\{ {{S_i}} \right\}}={E_s \over p_s}$, where $E_s$ is the expectation of service time under the condition that the considered update is not preempted by new updates and finally decoded successfully by the AP and $p_s$ denote the probability of such event. $E_s$ and $p_s$ can be evaluated as
\begin{equation}\label{ESeq}
{E_s} = {\sum\limits_{k = 0}^\infty  {{\varepsilon ^k}\left( {1 - \varepsilon } \right)\left( {1 - p} \right)} ^{k + 1}}\left( {k + 1} \right)M,
\end{equation}
\begin{equation}\label{PSeq}
{p_s} = {\sum\limits_{k = 0}^\infty  {{\varepsilon ^k}\left( {1 - \varepsilon } \right)\left( {1 - p} \right)} ^{k + 1}},
\end{equation}
where $p$ given in (\ref{p}) is the probability that an update being served is preempted by a new update and $k$ denotes the number of retransmission times. With the series expansion that ${1 \over {1 - x}} = \sum\limits_{n = 0}^\infty  {{x^n}} $ and ${1 \over {{{\left( {1 - x} \right)}^2}}} = \sum\limits_{n = 0}^\infty  {\left( {n + 1} \right){x^n}} $, we can solve $E_s$ and $p_s$ from (\ref{ESeq}) and (\ref{PSeq}) and they are given by $E_s={{\left( {1 - p} \right)\left( {1 - \varepsilon } \right)M} \over {{{\left[ {1 - \varepsilon \left( {1 - p} \right)} \right]}^2}}}$ and $p_s={{\left( {1 - p} \right)\left( {1 - \varepsilon } \right)} \over {1 - \varepsilon \left( {1 - p} \right)}}$. We can now derive the expectation of the service time for the retransmission scheme given by
\begin{equation}\label{Sire}
{\mathbb {E}\left\{ {{S_i}} \right\}}={M \over {1 - \varepsilon \left( {1 - p} \right)}}.
\end{equation}

To evaluate the expectation of $Y_i$, we use $K_i$ and $\hat K_i$ defined in Section III-B. The expectation of $K_i$ for the retransmission scheme can be evaluated as
\begin{equation}\label{Kieqre}
\begin{split}
\mathbb E\left\{ { {K_i}} \right\} &=\underbrace {\left(1-p\right)\left(1-\varepsilon\right)M}_{L_1} +\underbrace {\left(1-p\right)\varepsilon\left(M+\mathbb E\left\{ { \hat{K_i}} \right\}\right)}_{L_2}\\
&\quad+\underbrace {p\left(\mathbb E\left\{ {X_i\left| {X_i < m} \right.} \right\}+\mathbb E\left\{ { \hat{K_i}} \right\}\right)}_{L_3},
\end{split}
\end{equation}
where $L_1$ denote the case that the first generated update is not preempted and is decoded successfully by the AP. $L_2$ indicates the case that the update is not preempted and cannot be decoded successfully by the AP and thus evokes retransmission. $L_3$ shows the case that the first generated update is preempted by a new update. With the fact that $\mathbb E\left\{ { {K_i}} \right\}=\mathbb E\left\{ { {\hat K_i}} \right\}$ and the conditional expectation $\mathbb E\left\{ {X_i\left| {X_i < m} \right.} \right\}$ derived in (\ref{expect}), we can solve the expectation of $K_i$ from (\ref{Kieqre}) as
\begin{equation}\label{Kire}
\mathbb E\left\{ { {K_i}} \right\}= {p \over {\lambda \left( {1 - p} \right)\left( {1 - \varepsilon } \right)}}.
\end{equation}
With the expectation of $K_i$ for the retransmission scheme and $ \mathbb E\left\{ {{Z_i}} \right\} ={1\over \lambda}$, $\mathbb E\left\{ {{Y_i}} \right\}$ can be derived as
\begin{equation}\label{Yire}
\mathbb E\left\{ {{Y_i}} \right\} =\mathbb E\left\{ { {K_i}} \right\}+\mathbb E\left\{ { {Z_i}} \right\}={1-\varepsilon+p\varepsilon  \over {\lambda \left( {1 - p} \right)\left( {1 - \varepsilon } \right)}}.
\end{equation}
Next, we derive the expectation of $K_i^2$. Similar to that derived in Section III-B, we now have
\begin{equation}\label{Kire2eq}
\begin{split}
&\quad\left( {1 - p} \right)\left( {1 - \varepsilon } \right)\mathbb E\left\{ { {K_i^2}} \right\} \\
&=\left(1-p\right)M^2 +2\left(1-p\right)\varepsilon M \mathbb E\left\{ { {K_i}} \right\}+p\mathbb E\left\{ {X_i^2\left| {X_i < m} \right.} \right\}\\
&\quad+2p\mathbb E\left\{ { {K_i}} \right\}\mathbb E\left\{ {X_i \left| {X_i < m} \right.} \right\}. \\
\end{split}
\end{equation}
Substituting (\ref{expect}), (\ref{expect1}) and (\ref{Kire}) into (\ref{Kire2eq}), we can solve that
\begin{equation}
\mathbb E\left\{ { {K_i^2}} \right\} = {{2p\left( {1 - \varepsilon  + p\varepsilon } \right)} \over {{{\left[ {\lambda \left( {1 - p} \right)\left( {1 - \varepsilon } \right)} \right]}^2}}} - {{2M} \over {\lambda \left( {1 - p} \right)\left( {1 - \varepsilon } \right)}}.
\end{equation}
Then, $\mathbb E\left\{ { {Y_i^2}} \right\} $ can be calculated as
\begin{equation}\label{Yire2}
\begin{split}
\mathbb E\left\{ { {Y_i^2}} \right\} &= \mathbb E\left\{ { {K_i^2}} \right\}+2\mathbb E\left\{ { {K_i}} \right\}\mathbb E\left\{ { {Z_i}} \right\}+\mathbb E\left\{ { {Z_i^2}} \right\} \\
&=2{\left( {{{1 - \varepsilon  + p\varepsilon } \over {\lambda \left( {1 - p} \right)\left( {1 - \varepsilon } \right)}}} \right)^2} - {{2M} \over {\lambda \left( {1 - p} \right)\left( {1 - \varepsilon } \right)}}.
\end{split}
\end{equation}
Substituting (\ref{Sire}), (\ref{Yire}) and (\ref{Yire2}) into (\ref{delta}), we can derive the average AoI for the retransmission scheme given by
\begin{equation}
\Delta_{retr}={{1 - \varepsilon \exp \left( { - \lambda M} \right)} \over {\lambda \exp \left( { - \lambda M} \right)\left( {1 - \varepsilon } \right)}}.
\end{equation}
The optimal value of $m$ can be obtained by solving ${{d\Delta_{retr} } \over {dm}}=0$, which is characterized in the following equation
\begin{equation}
\lambda {T_u}\left( {1 - \varepsilon } \right) + {{\partial \varepsilon } \over {\partial m}}\left( {1 - {e^{ - \lambda {T_u}m}}} \right) = 0,
\end{equation}
where ${{\partial \varepsilon } \over {\partial m}}$ is given in (\ref{dedm}).

